Multi-Stage Cable Routing through Hierarchical Imitation Learning

We study the problem of learning to perform multi-stage robotic manipulation tasks, with applications to cable routing, where the robot must route a cable through a series of clips. This setting presents challenges representative of complex multi-stage robotic manipulation scenarios: handling deformable objects, closing the loop on visual perception, and handling extended behaviors consisting of multiple steps that must be executed successfully to complete the entire task. In such settings, learning individual primitives for each stage that succeed with a high enough rate to perform a complete temporally extended task is impractical: if each stage must be completed successfully and has a non-negligible probability of failure, the likelihood of successful completion of the entire task becomes negligible. Therefore, successful controllers for such multi-stage tasks must be able to recover from failure and compensate for imperfections in low-level controllers by smartly choosing which controllers to trigger at any given time, retrying, or taking corrective action as needed. To this end, we describe an imitation learning system that uses vision-based policies trained from demonstrations at both the lower (motor control) and the upper (sequencing) level, present a system for instantiating this method to learn the cable routing task, and perform evaluations showing great performance in generalizing to very challenging clip placement variations. Supplementary videos, datasets, and code can be found at https://sites.google.com/view/cablerouting.

==> sections/bio.tex <==
\vspace{11pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{rss2021/figs/jianlan_luo.jpg}}]{Jianlan Luo(M’20)} received the M.S. degree and the Ph.D. degree in Computer Science and Mechanical Engineering from the University of California, Berkeley, CA, USA in 2020.
He is currently a postdoctoral researcher in the Department of Electrical Engineering and Computer Sciences at UC Berkeley. He was a researcher at the robotics division of Google [X] lab from 2020-2022. 
He is broadly interested in topics intersecting between robotics, machine learning, and optimal control; focuses on developing robust autonomous systems that can solve dynamic tasks.
 

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Charles.jpg}}]{Charles Xu} 
is currently working towards his BS degree in Electrical Engineering and Computer Science at UC Berkeley, CA, USA. He is advised by Sergey Levine at the Berkeley AI Research Lab (BAIR). His research interests lie at the intersection of machine learning and industrial robotics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/young.jpg}}]{Xinyang Geng}  received a B.A degree in computer science and statistics from UC Berkeley in 2017, where he is currently working towards the Ph.D. degree in computer science, advised by Professor Sergey Levine.
His interests lie in the intersection between large-scale self-supervised learning and decision-making. Specifically, his research focuses include machine learning, deep reinforcement learning, and model-based optimization.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{rss2021/figs/gilbert.jpg}}]{Gilbert Feng} received the B.S. degree in Electrical Engineering and Computer sciences from the University of California, Berkeley, Berkeley, CA, USA, in 2022.
His research interests include applications of imitation learning and reinforcement learning toward control of robotic systems, with a focus on morphology and task generalization in real-world environments.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{rss2021/figs/kuan_fang.jpg}}]{Kuan Fang(M’21)} received the M.S. degree and the Ph.D. degree in Electrical Engineering from Stanford University, Stanford, CA, USA in 2017 and 2021, respectively. He is currently a postdoctoral researcher in the Department of Electrical Engineering and Computer Sciences at UC Berkeley. His research interest lies at the intersection of robotics, computer vision, and machine learning. Specifically, he develops scalable data-driven methods for robots to solve diverse and complex tasks in unstructured environments.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{rss2021/figs/Liam_photo.jpg}}]{Liam Tan}
is currently working towards his BS degree in Computer Science and Math at UC Berkeley, CA, USA. He is advised by Sergey Levine at the Berkeley AI Research Lab (BAIR). He is interested in large-scale pretraining, robot learning, reinforcement learning, and controls.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/stefan.jpg}}]{Stefan Schaal} received his Ph.D. from the Technical University of Munich in Mechanical Engineering and Artificial Intelligence in 1991; then a postdoctoral fellow at the Department of Brain and Cognitive Sciences and the Artificial Intelligence Laboratory at MIT, an Invited Researcher at the ATR Human Information Processing Research Laboratories in Japan, and an Adjunct Assistant Professor at the Georgia Institute of Technology and at the Department of Kinesiology of the Pennsylvania State University. He also held an appointment as Head of the Computational Learning Group during an international Japanese ERATO project, the Kawato Dynamic Brain Project (ERATO/JST). In 1997 Stefan became a Professor of Computer Science, Neuroscience, and Biomedical Engineering at the University of Southern California, where he advanced to the rank of full professor with tenure. Stefan is a Founding Director of the Max-Planck-Institute for Intelligent Systems in Germany where he led the Autonomous Motion Department for several years. Stefan is currently the Chief Science Officer at Intrinsic, a new robotics subsidiary of Alphabet [Google].

Stefan’s research interests include topics of statistical and machine learning, neural networks and artificial intelligence, computational neuroscience, functional brain imaging, nonlinear dynamics, nonlinear control theory, and robotics and biomimetic robotics. He is a co-founder of the "IEEE/RAS International Conference and Humanoid Robotics" and a co-founder of "Robotics Science and Systems". Stefan served as Program Chair at these conferences and he was the Program Chair of "Simulated and Adaptive Behavior" (SAB 2004) and the "IEEE/RAS International Conference on Robotics and Automation" (ICRA 2008), the largest robotics conference in the world. Stefan is has also been an Area Chair at "Neural Information Processing Systems" (NeurIPS) and served as Program Committee Member of the "International Conference on Machine Learning" (ICML). Stefan has served on the editorial board of the journals "Neural Networks", "International Journal of Humanoid Robotics", and "Frontiers in Neurorobotics". Stefan is a member of the German National Academic Foundation (Studienstiftung des Deutschen Volkes), the Alexander von Humboldt Foundation, the Society for Neuroscience, the Society for Neural Control of Movement, the AAAS, and a Fellow of the IEEE. Stefan initiated and maintained the largest robotics email list in the world — robotics-worldwide — and contributed to the organization and reviewing of several dozens of conferences, journals, and US and European funding organizations.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{rss2021/figs/sergey.jpg}}]{Sergey Levine} received a BS and MS in Computer Science from Stanford University in 2009, and a Ph.D. in Computer Science from Stanford University in 2014. He joined the faculty of the Department of Electrical Engineering and Computer Sciences at UC Berkeley in fall 2016, where he is currently an associate professor. His work focuses on machine learning for decision-making and control, with an emphasis on deep learning and reinforcement learning algorithms. Applications of his work include autonomous robots and vehicles, as well as applications in other decision-making domains. His research includes developing algorithms for end-to-end training of deep neural network policies that combine perception and control, scalable algorithms for inverse reinforcement learning, deep reinforcement learning algorithms, and more.
\end{IEEEbiography}

